Two-Pass End-to-End Speech Recognition

The requirements for many applications of state-of-the-art speech recognition systems include not only low word error rate (WER) but also low latency. Specifically, for many use-cases, the system must be able to decode utterances in a streaming fashion and faster than real-time. Recently, a streaming recurrent neural network transducer (RNN-T) end-to-end (E2E) model has shown to be a good candidate for on-device speech recognition, with improved WER and latency metrics compared to conventional on-device models [1]. However, this model still lags behind a large state-of-the-art conventional model in quality [2]. On the other hand, a non-streaming E2E Listen, Attend and Spell (LAS) model has shown comparable quality to large conventional models [3]. This work aims to bring the quality of an E2E streaming model closer to that of a conventional system by incorporating a LAS network as a second-pass component, while still abiding by latency constraints. Our proposed two-pass model achieves a 17%-22% relative reduction in WER compared to RNN-T alone and increases latency by a small fraction over RNN-T.

==> results_ahvsime.tex <==
\section{Results \label{sec:results}}

\subsection{2nd Beam Search}

Table \ref{table:2ndbeam} shows the results running the LAS decoder in the 2nd
beam-search mode.
%
For comparison, the table also shows two baselines \texttt{B0-B1}, namely an
RNN-T only and a LAS-only model.
%
All results are obtained with fixed beam-size of $H=8$ hypotheses.

Experiment \texttt{E0} indicates that when the encoder is held fixed and
initialized from an RNN-T model, the LAS decoder performs worse than a LAS-only
model with a dedicated encoder (\texttt{B1}), demonstrating the challenges in
sharing a single encoder with different types of decoders by adapting the LAS
decoder alone.
%
When we jointly train the encoder and both decoders in a model initialized from
\texttt{E0}, the model quality (\texttt{E1}) improved in both SU and LU over
\texttt{E0}.
Overall we find that 2nd beam search improves over RNN-T (\texttt{B0}) on SU but
degrades on LU, a common issue with attention models for long utterances
\cite{Jan15}.

\begin{table} [h!]
  \centering
  \caption{WER Results, LAS Beam Search.}
  \begin{tabular}{|c||c|c|c|} \hline
    Exp-ID & Model & SU & LU \\ \hline
    \textit{B0} & RNN-T & 6.9 & 4.3 \\ \hline
    \textit{B1} & LAS-only & 5.4 &  4.6  \\ \hline
    \textit{E0} & Frozen Shared Enc & 6.3 & 5.1 \\ \hline
    \textit{E1} & Deep Finetuned & 6.0 & 4.7 \\ \hline
  \end{tabular}
  \label{table:2ndbeam}
  \vspace{-0.1in}
\end{table}

In addition, we also study the change in estimated latency and model quality change as
the LAS decoder beam size is varied, as shown in Table \ref{table:2ndbeamops}.
The table indicates that while SU and LU performance remains stable, contacts biasing
WER degrades significantly with a smaller beam.
%
Contextual biasing is very challenging with E2E models, which do poorly with proper noun
recognition \cite{Pundak18}.
%
It is critical to have enough number of hypotheses in a beam search to ensure
that proper noun biasing phrases do not fall off the beam.
%
Hence biasing requires the LAS decoder to run with a beam of 8, which increases
two-pass latency by over 700ms, which is far above our allowable limit.

\begin{table} [h!]
  \centering
  \caption{LAS Performance vs. Beam Size.}
  \begin{tabular}{|c||c|c|c|c|} \hline
    Beam Size & SU & LU & Contacts & Latency (ms)  \\ \hline
    2 & 6.1 & 4.8 & 9.4 & 184.8 \\ \hline
    4 & 6.0 & 4.7 & 7.7 & 369.6  \\ \hline
    8 & 6.0 & 4.7 & 6.8 & 739.2 \\ \hline
  \end{tabular}
  \label{table:2ndbeamops}
    \vspace{-0.1in}
\end{table}


\subsection{Rescoring}

The RNN-T-only model (\texttt{B0}) has an oracle WER of 2.2 on SU and 1.5 on
LU, much lower than its WER of 6.9 on SU and 4.3 on LU.
%
This motivates us to explore rescoring RNN-T hypothesis with the LAS decoder.
%
Table \ref{table:rescoring} compares the performance of running LAS with beam
search (\texttt{E1}) to with rescoring (\texttt{E2}).
%
The table shows that rescoring takes a small hit in WER on SU compared to beam
search, probably because the first-pass RNN-T decoder, with a much higher SU WER
of 6.9 (\texttt{B0}), generates a set of hypotheses with slightly lower quality
than those generated by the LAS decoder during beam search.
%
However, rescoring's quality on LU is much better than that of beam search,
likely because RNN-T (\texttt{B0}) performs much better on longer utterances
compared to LAS.
%
Overall, LAS rescoring not only improves SU WER significantly upon the first
pass RNN-T, but also improves WER for LU, demonstrating that rescoring is able
to combine the strengths of RNN-T and LAS.

\begin{table} [h!]
  \centering
  \caption{WER results, LAS Rescoring.}
  \begin{tabular}{|c||c|c|c|} \hline
    Exp-ID & Decoding & SU & LU \\ \hline
    \textit{B0} & RNN-T & 6.9 & 4.3 \\ \hline
    \textit{B1} & LAS-only & 5.4 &  4.6 \\ \hline
    \textit{E1} & Beam Search & \textbf{6.0} & 4.7 \\ \hline
    \textit{E2} & Rescoring & 6.2 & \textbf{4.0} \\ \hline
  \end{tabular}
  \label{table:rescoring}
    \vspace{-0.1in}
\end{table}


Next, Table \ref{table:2ndrescops} shows WER on SU, LU and a contacts biasing
set, as well as the latency, as the number of rescoring beams is
varied.
%
For these experiments, the 1st-pass RNN-T model is run with a fixed beam size of 8.
%
The table indicates that we can prune the number of rescored hypotheses to 4, with no
loss in accuracy on any test set.
%
Overall, rescoring 4 hypotheses requires half the latency compared to the
2nd beam search decoding with 8 hypotheses in Table \ref{table:2ndbeamops}.


%
Since rescoring gives us the best tradeoff between quality and computation cost,
we will focus only on rescoring and present further improvements in the next
section.

\begin{table} [h!]
  \centering
  \caption{LAS Performance vs. Rescoring Beam Size.}
  \begin{tabular}{|c||c|c|c|c|} \hline
    Rescoring Beam & SU & LU & Contacts & Latency (ms)  \\ \hline
    2 & 6.2 & 4.0 & 7.5 & 184.8  \\ \hline
    4 & 6.2 & 4.0 & 7.1 & \textbf{369.6} \\ \hline
    8 & 6.2 & 4.0 & 7.1 & 739.2 \\ \hline
  \end{tabular}
  \label{table:2ndrescops}
    \vspace{-0.2in}
\end{table}


\subsection{Further Rescoring Improvements}

\subsubsection{Adaptive Beam}

To bridge the gap between two-pass 2nd beam search vs. rescoring on SU, we explore increasing the first-pass RNN-T beam size.
%
Table \ref{table:adaptive} shows that as beam size is increased (\texttt{E2-E4}), both WER and oracle WER improve, but at a cost of increased first-pass computation cost.
%
To address this, we look at an adaptive beam search strategy \cite{Lowerre76}. Specifically, we prune first-pass beam candidates if the they are too far in threshold from the current best candidate, where the threshold optimizes first-pass latency following \cite{Ryan19}.
%
The table shows that with an adaptive beam (\texttt{E5}), we can achieve similar WER to a fixed but large beam.

\begin{table} [h!]
  \centering
  \caption{Two-pass rescoring with fixed vs. adaptive beam.}
  \begin{tabular}{|c||c|c|c|c|c|} \hline
    Exp-ID & First-pass &  \multicolumn{2}{c}{SU} &  \multicolumn{2}{c}{LU}  \\
           & Max Beam Size & WER & oracle & WER & oracle    \\ \hline
    \textit{E2} & Fixed, 8 & 6.2 & 2.2 & 4.0 & 1.5  \\ \hline
    \textit{E3} & Fixed, 10 & 6.1 & 2.1 & 4.0 & 1.4 \\ \hline
    \textit{E4} & Fixed, 16 & 6.1 & 1.9 & 4.0 & 1.3 \\ \hline
    \textit{E5} & Adaptive, 10 & 6.1 & 2.1 & 3.9 & 1.4  \\ \hline
  \end{tabular}
  \label{table:adaptive}
    \vspace{-0.1in}
\end{table}

The adaptive-beam also has the additional benefit that it generates a lattice to use for rescoring, rather than an N-best list. A lattice is less dense than an N-best list, which should improve rescoring latency. As a reminder, latency in Equation \ref{eq:latency} is now calculated by looking at the total arcs in the lattice.
%
Two-pass rescoring is run on the top 4 hypotheses from first pass decoding in
both cases, following results from Table \ref{table:2ndrescops}.
%
Table ~\ref{table:adaptiveops} show that with an adaptive beam and lattice rescoring, we get a 2X reduction in latency compared to a fixed beam with N-best rescoring.
%
Overall, the two-pass rescoring decoder with adaptive beam fits within our 200ms latency budget.

\begin{table} [h!]
  \centering
  \caption{LAS Performance vs. Rescoring Beam Size.}
  \begin{tabular}{|c||c|c|c|c|} \hline
    Strategy & SU & LU & Contacts & Latency (ms)  \\ \hline
    1st-pass Fixed & 6.2 & 4.0 & 7.1 & 369.6 \\
    N-best Rescoring &     &     &      &   \\ \hline
    1st-pass Adaptive & 6.1 & 3.9 & 7.1 & \textbf{171.6}  \\
    Lattice Rescoring &     &     &      &   \\ \hline
  \end{tabular}
  \label{table:adaptiveops}
    \vspace{-0.1in}
\end{table}

\subsubsection{MWER}

Finally, we report two-pass results after MWER training our model.  Table
\ref{table:embr} shows that MWER improves rescoring WER for both SU and LU by
8\% relative. Overall, the two-pass rescoring model gives a 19\% relative reduction in both SU and LU 
%and brings the SU WER close to that of a standalone LAS model.
%\TS{i'm leaving beam search out it doesnt even fit within the latency budget it seems distracting to put in here.}

\begin{table} [h!]
  \centering
  \caption{Two-pass rescoring results after MWER training.}
  \begin{tabular}{|c||c|c|c|c|} \hline
    Exp-ID & Model & SU & LU & Contacts \\ \hline
    \textit{B0} & RNN-T only & 6.9 & 4.3 & \\ \hline
    \textit{E5} & No MWER & 6.1 & 3.9 & 7.1 \\ \hline
    \textit{E6} & MWER & \textbf{5.6} & \textbf{3.5} & \\ \hline
  \end{tabular}
  \label{table:embr}
    \vspace{-0.1in}
\end{table}

\subsection{Comparison To Large Conventional Model}
% https://furball.corp.google.com/project/load?projectId=122622519#!tab=asr_sxs_analysis_ipynb
A goal of our work is to achieve in an E2E system with comparable performance to
a large conventional model \cite{Golan16}. In this light, we compare the
performance of our proposed two-pass rescoring model to a large conventional
model through a ``side-by-side'' (SxS) evaluation with previously unseen utterances.
In this experiment, each utterance is transcribed by both the conventional and
two-pass models. We collect 500 utterances where the transcription differs
between the two models, and send these utterances to be rated by two human
transcribers. Each transcript is rated as either a win by two-pass over the
conventional model (only two-pass is correct), a loss in two-pass over the
conventional model (only the conventional model is correct), or neutral (both models are correct or incorrect).
Unlike automatic WER evaluations, this side-by-side evaluation allows raters to decide that two different transcripts are both correct; this sometimes leads to different conclusions
than an automatic evaluation would.
We report the following statistics to quantitatively evaluate the SxS:
\begin{itemize}
\item Changed: \% of utterancs in which the two models produced different hypotheses
\item Wins: \# of utts the two-pass hypothesis is correct and conventional model is incorrect
\item Losses: \# of utts the two-pass hypothesis is incorrect and conventional model is correct
\item Neutral: \# of utts the two-pass and conventional model are both correct or incorrect
\item p-Value: Statical significance of WER change with two-pass compared to conventional model
\end{itemize}

Table \ref{table:sxs} shows that the two-pass model changes about 13\% of traffic. The two-pass model has slightly more losses (61) than wins (48) compared to the conventional model, but the majority of the hypotheses have a neutral rating (391) between the two systems. Overall, the p-Value shows the performance difference between the two models is statistically insignificant.

\begin{table}[h!]
  \centering
  \caption{SxS results for Conventional vs. Two-pass}
  \begin{tabular}{|c|c|c|c|c|} \hline
    Changed (\%) & Win & Loss & Neutral & p-Value \\ \hline
    13.2 & 48 & 61 & 391 & 10.0\%-20.0\%  \\ \hline
  \end{tabular}
  \label{table:sxs}
    \vspace{-0.1in}
\end{table}


A further analysis of errors is shown in Table \ref{table:wins_and_losses}. The two-pass model is trained with an order of magnitude less text-only data compared to the conventional model, and thus loses on proper nouns and in sentences requiring a stronger LM. On the contrary, since the two-pass model is trained in the written domain and learns text normalization implictly, it wins in this area compared to the conventional model which has a separate rule-based text-norm step.

\begin{table} [h!]
\centering
\caption{Analysis of Errors of Conventional vs. Two-Pass Model.}
\begin{tabular}{|c||c|c|c|} \hline
 & Category & Conventional &  Two-Pass \\ \hline
Loss & Proper Noun & \footnotesize{alice's restaurant} & \footnotesize{\red{allison's restaurant}} \\
& weak LM & \footnotesize{47-in sony plasma tv} & \footnotesize{47-in sony \red{pricing} tv} \\ \hline
 Win & Text-norm & \footnotesize{www nytimes.com} & \footnotesize{\green{www.nytimes.com}} \\
& Text-norm & \footnotesize{john smiths office} & \footnotesize{john \green{smith's} office} \\ \hline
\end{tabular}
\vspace{-0.1 in}
\label{table:wins_and_losses}
\end{table}

